Efficient Diffusion Transformer Policies with Mixture of Expert Denoisers for Multitask Learning

Diffusion Policies have become widely used in Imitation Learning, offering several appealing properties, such as generating multimodal and discontinuous behavior. As models are becoming larger to capture more complex capabilities, their computational demands increase, as shown by recent scaling laws. Therefore, continuing with the current architectures will present a computational roadblock. To address this gap, we propose Mixture-of-Denoising Experts (MoDE) as a novel policy for Imitation Learning. MoDE surpasses current state-of-the-art Transformer-based Diffusion Policies while enabling parameter-efficient scaling through sparse experts and noise-conditioned routing, reducing both active parameters by 40% and inference costs by 90% via expert caching. Our architecture combines this efficient scaling with noise-conditioned self-attention mechanism, enabling more effective denoising across different noise levels. MoDE achieves state-of-the-art performance on 134 tasks in four established imitation learning benchmarks (CALVIN and LIBERO). Notably, by pretraining MoDE on diverse robotics data, we achieve 4.01 on CALVIN ABC and 0.95 on LIBERO-90. It surpasses both CNN-based and Transformer Diffusion Policies by an average of 57% across 4 benchmarks, while using 90% fewer FLOPs and fewer active parameters compared to default Diffusion Transformer architectures. Furthermore, we conduct comprehensive ablations on MoDE's components, providing insights for designing efficient and scalable Transformer architectures for Diffusion Policies. Code and demonstrations are available at https://mbreuss.github.io/MoDE_Diffusion_Policy/.

==> chapters/old_method_outdated.tex <==
\section{Method}
%\begin{figure}
%    \centering
%    \vspace{-5pt} 
%    \includegraphics[width=0.95\columnwidth]{figures/images/Denoising_fig.pdf}
    % \vspace{-20pt} 
%    \caption{Denoising Process of MoDE with sparse activated experts. Our novel noise-only routing strategy activates %topk experts based on the current noise level of the diffusion process.  }
%    \label{fig: denoising process}
%\end{figure}

In this section, we introduce \gls{mode}, our novel MoE Diffusion Policy. 
First, we formulate the problem of learning a policy for \gls{gcil}.
\textcolor{brown}{
Next, we summarize the framework used in Diffusion Policies and then introduce our \gls{mode} architecture with our novel noise-conditioned routing and noise-conditioned self-attention that enable efficient policy design. Finally, we explain our expert caching mechanism for efficient inference.
}

\subsection{Problem Formulation}

We consider the problem of learning a language-conditioned policy $\pi_{\theta}(\act | \state, \goal)$ given a dataset of robot demonstrations $\Tset$.
The policy predicts a sequence of future actions $\act = (\act*,\ldots,\act*[i+j-1])$ of length $j$, conditioned on the history of state embeddings $\state = (\state*[i-h +1],\ldots, \state*[i])$ of length $h$ and a desired goal $\goal$. 
The dataset contains $\tau \in \Tset$ trajectories, where trajectory consists of a sequence of triplets of state, actions, and goal $(\state[i], \act*[i], \goal)$.
$\goal$ is a language instruction. 
Our policy is trained to maximize the log-likelihood of the action sequence given the context of state history and goal:
\begin{align}
    \mathcal{L}_{\text{IL}} = \mathbb{E} \left[ \sum_{(\state,\act, \goal) \in \Tset} \log \p{\pi_\theta}{\act | \state, \goal}  \right].
\end{align}



\subsection{Diffusion Policy}

\gls{mode} uses the continuous-time diffusion model of EDM~\citep{karras2022elucidating} as a policy representation.
Diffusion models are a type of generative model for generating data by initially adding noise through Gaussian perturbations and then reversing this process. 
\gls{mode} applies the score-based diffusion model to represent the policy $\pi_{\theta}(\act | \state, \goal)$.
The perturbation and inverse process can be described using a stochastic differential equation:
\begin{equation}
\label{eq: conditional Karras Song SDE}
\begin{split}
\diff \act  =  \big( \beta_t \sigma_t - \dot{\sigma}_t  \big) \sigma_t \nabla_a \log p_t(\act | \state, \goal) dt + \sqrt{2 \beta_t} \sigma_t d\omega_t,
 \end{split}
\end{equation}
where $\beta_t$ controls the noise injection, $d\omega_t$ refers to infinitesimal Gaussian noise, and $p_t(\act | \state, \goal)$ is the score function of the diffusion process, that moves samples away from regions of high-data density in the forward process.
To generate new samples from noise a neural network is trained to approximate the score function $\nabla_{\act} \log p_t(\act |\state, \goal)$ via Score matching (SM)~\citep{6795935}
\begin{equation}
\label{eq: SM loss}
    \mathcal{L}_{\text{SM}} = \mathbb{E}_{\mathbf{\sigma}, \act, \boldsymbol{\epsilon}} \big[ \alpha (\sigma_t) \newline  \| D_{\theta}(\act + \boldsymbol{\epsilon}, \state, \goal, \sigma_t)  - \act  \|_2^2 \big],
\end{equation}
where $D_{\theta}(\act + \boldsymbol{\epsilon}, \state, \goal, \sigma_t)$ is the trainable neural network.
During training, we sample noise from a training distribution and add it to an action sequence.
The network predicts the denoised actions and computes the SM loss. 
% For our noise distribution, we consider a LogLogistic distribution similar to prior work~\citep{reuss2023goal}.

After training, we can generate a new action sequence starting from random noise by approximating the reverse SDE or related ODE in discrete steps using numerical ODE integrators. 
Therefore, we sample noise from the prior $\act*[T] \sim \mathcal{N}(\mathbf{0}, \sigma_T^2 \mathbf{I})$ and iteratively denoise it.
\gls{mode} uses the DDIM-solver, a numerical ODE-solver designed for diffusion models~\citep{song2021denoising}, that allows fast denoising of actions in a few steps.
\gls{mode} uses $10$ denoising steps in all our experiments. 


\subsection{Mixture-of-Experts Denoising} 

We now present the details of \gls{mode}'s noise-conditioned expert routing.
\textcolor{brown}{An overview of \gls{mode} and the expert-routing is shown in \autoref{fig: mode architecture overview}.}
For language conditioning, \gls{mode} uses a frozen CLIP language encoder model to generate a single latent goal vector. 
To encode images, \gls{mode} uses FiLM-conditioned ResNets-18.  
Let $\bf{X} \in \mathbb{R}^{\text{tokens} \times D}$ be a sequence of input tokens of dimension $D$, and $\sigma_t$ be the noise level. 
Let $\phi(\sigma_t)$ encode the noise level into a token using a linear projection layer, and let $\bf{X}$ also contain $\phi(\sigma_t)$ as a token.  
$\text{MoDE}(\bf{X}, \phi(\sigma_t))$ is a composition of $L$ transformer blocks which we will now describe in detail.

Each transformer block $f^i$ takes $\phi(\sigma_t)$ as input as well. 
We now define each block $f^i$ as a composition of a self-attention (SA) layer and an $\text{MoE}$ layer,
\begin{equation}
    f^i(\bf{X}, \phi(\sigma_t)) = \text{MoE}(\text{SA}(\hat{\bf{X}}) + \bf{X}, \phi(\sigma_t)) + \bf{X}.    
\end{equation}
We add the noise token, $\phi(\sigma_t)$ to all the tokens in $\bf{X}$ before computing the self-attention as done in \citep{hatamizadeh2023diffit}. 
\textcolor{brown}{This addition acts as a noise-aware positional embedding, allowing each token to adapt its attention patterns based on the current denoising phase. 
This enables better learning of the denoising, without adding any parameters or novel model parts.}
\begin{equation}
    \hat{\bf{X}} = \phi(\sigma_t) + \bf{X},
\end{equation}
and following \citep{vaswani2017attention},
\begin{equation}
    \text{SA}(\hat{\bf{X}}) = \text{softmax}(\frac{1}{\sqrt{D}} [\hat{\bf{X}}W_Q][\hat{\bf{X}}W_K]^T)[\hat{\bf{X}}W_V].
\end{equation}
Given $N$ experts $\{\bf{E_i}\}_{i=1}^N$, we define the sparse MoE layer as
\begin{equation}
    \text{MoE}(\bf{X}, \phi(\sigma_t))= \sum_{i=1}^N \bf{R}(\phi(\sigma_t)) \bf{E}_i(\bf{X}),
\end{equation}
where, the routing function $\bf{R}(\cdot): \mathbb{R}^{\text{tokens} \times D} \rightarrow \mathbb{R}^{\text{tokens} \times N}$. 
Our noise-only conditioned routing function is defined as
\begin{equation}
    \bf{R}(\phi(\sigma_t)) = \text{topk}(\text{softmax}(\phi(\sigma_t)W_R), \textit{k})
\end{equation}
\textcolor{brown}{Contrast to standard MoE of the LLM Literature, \gls{mode} employs a novel noise-only routing strategy adapted for Diffusion Policies. 
In \gls{mode}'s routers experts are chosen based on the current noise level of the denoising process.
Thus, our model learns specialist experts for different noise regions and can employ fused expert caching as described in \autoref{sec:router_expert_caching}.}
While $\text{topk}$ typically varies across different \gls{moe} implementations, we use multinomial sampling. 
Where we sample without replacement $\textit{k}$ elements according to their probabilities given by $\text{softmax}(\phi(\sigma_t)W_R)$. 
We set all non-chosen elements to $0$. 
Since sampling is a non-differentiable process, scaling the expert outputs by the routing probability, $\bf{E}_i(\bf{X})$ is needed to pass gradients to the routing function. 
In addition, we optimally re-normalize the chosen $\textit{k}$ elements probabilities. 
After the final layer, we use a linear projection layer to get the denoised action sequence.

In addition, to mitigate expert collapse, we adopt an additional loss function ($LB$) that regularizes the router called load balancing ~\citep{fedus2022switch}. Here for a given expert $E_i$, we compute the fraction of the tokens that were routed to it, under $\text{topk}$ being an $\arg \max$ function, and we scale that by the average probability of routing to $E_i$ across all tokens in a batch $\mathcal{B}$. 
\begin{equation}
    LB(\sigma_t) = N \sum_{n=1}^N \frac{1}{|\mathcal{B}|}(\sum_{i=1}^{|\mathcal{B}|}\mathbbm{1}\{\bf{R}(\phi(\sigma_{t_i}))_n > 0\})\frac{1}{|\mathcal{B}|}(\sum_{i=1}^{|\mathcal{B}|}\text{softmax}(\phi(\sigma_{t_i})W_R)_n)
\end{equation}
We use $\gamma=0.01$ for the load-balancing loss. 



\subsubsection{Router and Expert Caching}
\label{sec:router_expert_caching}
\begin{figure*}[t]
\hspace{-1em}
    \centering
    \includegraphics[width=0.75\columnwidth]{figures/images/caching.pdf}
    \caption{Visualized Expert Utilization. 
    The top row depicts the chosen experts ($k=2$) for different noise levels. Focusing on just time step $i$, we know that the routing is deterministic at each time step. Therefore, we can create a more efficient network that minimizes the overhead of a traditional MoE by creating fused experts which is depicted in the second row.}
    \label{fig:caching}
\end{figure*}
\textcolor{orange}{To make our method more efficient, we exploit the fact that our MoE is noise-conditioned, meaning that at each noise level, the routing path is deterministic and can be precomputed. By doing so, we can determine the chosen experts ahead of time for each noise level. \autoref{fig:caching} illustrates this process. This allows us to fuse the selected expert MLPs into a single, composite MLP, effectively reducing the computation cost.}

\textcolor{orange}{Instead of looping through each expert individually, this fused expert MLP can run in parallel forward pass, which substantially decreases the overall latency of the network. 
By eliminating the need for dynamically invoking each expert, we not only save time but also streamline memory access patterns, reducing the overhead typically associated with routing decisions in a traditional MoE setup. 
Our caching strategy reduces the FLOPs overhead by over 87$\%$ compared to standard MoE rollouts and makes it two times faster during inference.
}


\subsection{Generalist Policy Pre-Training}
\label{sec:generalist-pretraining}
\textcolor{purple}{We pretrain \gls{mode} on a diverse mix of multi-robot datasets curated from the OXE dataset \cite{open_x_embodiment_rt_x_2023}. 
We choose a subset of 6 datasets that consist of more than 196k trajectories of various robots in diverse settings. 
We pretrain \gls{mode} for 300k steps using a small cluster with 6 GPUs for 3 days. 
For finetuning we freeze the pretrained routers in each layer and only finetune the other model components. 
An detailed overview of our pretraining mix and used datasets is given in \autoref{sec:pretraining-details} of the Appendix.
Additional experiments against other generliast policies is provided in }

==> figures/experiments/MoDE_Performance_Speed.tex <==
\begin{tikzpicture}
\definecolor{crimson}{RGB}{214,39,40}
\definecolor{darkgray}{RGB}{176,176,176}
\definecolor{darkorange}{RGB}{255,127,14}
\definecolor{darkturquoise}{RGB}{23,190,207}
\definecolor{forestgreen}{RGB}{44,160,44}
\definecolor{goldenrod}{RGB}{188,189,34}
\definecolor{gray}{RGB}{127,127,127}
\definecolor{mediumpurple}{RGB}{148,103,189}
\definecolor{orchid}{RGB}{227,119,194}
\definecolor{sienna}{RGB}{140,86,75}
\definecolor{steelblue}{RGB}{31,119,180}

% First plot: Average Score
\begin{axis}[
    ybar,
    name=score,
    width=3.5cm,
    bar width=15pt,
    xtick=data,
    ylabel={\small Avg. Score ($\%$)},
    ymajorgrids,
    ymin=80,
    ymax=86,
    enlarge x limits=0.3,
    nodes near coords,
    every node near coord/.append style={font=\scriptsize},
    xticklabels={\small MoDE, \small BESO},
    xtick={0, 1},
    ytick={80, 84},
]

% MoDE
\addplot [ybar, draw=steelblue,
    line width=.2mm,
    fill opacity=0.7,
    fill=steelblue,
    bar shift=0pt,
] coordinates {
    (0, 84.03)
};

% BESO
\addplot [ybar, draw=forestgreen,
    line width=.2mm,
    fill opacity=0.7,
    fill=forestgreen,
    bar shift=0pt,
] coordinates {
  (1, 82.35)
};

\end{axis}

\hspace{0.5cm}

% Second plot: Inference Speed
\begin{axis}[
    width=3.5cm,
    name=speed,
    at=(score.right of south east),
    anchor=left of south west,
    bar width=15pt,
    ylabel={\small Inf. Speed (ms)},
    ymajorgrids,
    ymin=0, ymax=200,
    enlarge x limits=0.3,
    nodes near coords,
    every node near coord/.append style={font=\scriptsize},
    ybar,
    xticklabels={\small MoDE, \small BESO},
    xtick={0, 1},
    ytick={0,100,200}
]

% MoDE Inference Speed
\addplot [ybar, draw=steelblue,
    line width=.2mm,
    fill opacity=0.7,
    fill=steelblue,
    bar shift=0pt,
] coordinates {
    (0, 100)
};

% BESO Inference Speed
\addplot [ybar, draw=forestgreen,
    line width=.2mm,
    fill opacity=0.7,
    fill=forestgreen,
    bar shift=0pt,
] coordinates {
    (1, 150)
};

\end{axis}

\end{tikzpicture}

==> figures/experiments/environments_overview.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.22\textwidth}  % Adjust width to fit within a column
        \centering
        \includegraphics[width=\linewidth]{figures/images/CALVIN_ABCD.pdf}
        \caption{CALVIN}
        \label{fig:env1}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.26\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/bet_block_push.pdf}
        \caption{Block Push}
        \label{fig:env2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/rely_kitchen.pdf}
        \caption{Relay Kitchen}
        \label{fig:env3}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.21\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/images/libero_long.pdf}
        \caption{LIBERO-Long}
        \label{fig:env4}
    \end{subfigure}
    \caption{Overview of the environments used to test MoDE. (a) CALVIN contains four different settings (A,B,C,D) with different configurations of slides, drawers and textures. (b) Block-Push and (c) Relay-Kitchen are two state-based environment. For (d) LIBERO-10 we show an example task used in the challenge consisting of $10$ long horizon tasks in different settings.}
    \label{fig:three-environments}
\end{figure*}


==> figures/experiments/n_expert_scaling.tex <==
\begin{tikzpicture}
\definecolor{crimson}{RGB}{214,39,40}
\definecolor{darkgray}{RGB}{176,176,176}
\definecolor{darkorange}{RGB}{255,127,14}
\definecolor{darkturquoise}{RGB}{23,190,207}
\definecolor{forestgreen}{RGB}{44,160,44}
\definecolor{goldenrod}{RGB}{188,189,34}
\definecolor{gray}{RGB}{127,127,127}
\definecolor{mediumpurple}{RGB}{148,103,189}
\definecolor{orchid}{RGB}{227,119,194}
\definecolor{sienna}{RGB}{140,86,75}
\definecolor{steelblue}{RGB}{31,119,180}
% First plot: Average Score

\begin{axis}[
    name=abc,
    width=4cm,
    ylabel=Performance,
    ylabel style={at={(axis description cs:-0.15,.5)},anchor=south},
    xlabel=Number Experts,
    ymin=0, ymax=5,
    xmin=4, xmax=8,
    xtick={4,6,8},
    xticklabels={4,6,8},
    yticklabels={0,1,2,3,4,5},
    grid=both,
    grid style={dashed},
    nodes near coords,
    point meta=explicit symbolic,
    enlarge x limits=0.3,
    nodes near coords,
    every node near coord/.append style={font=\small},
    legend style={at={(0.5,-0.45)},anchor=north,legend columns=2}
]
        \addplot+[steelblue, sharp plot, no markers, mark options={solid}, line width=1pt] coordinates {

            (4, 0.87)
            (5, 0.87)
        };
        \addplot+[crimson, sharp plot, no markers, mark options={solid}, forget plot, line width=1pt] coordinates {
            (3, 0.95)
            (4, 0.95)
            (5, 0.94)
            (6, 0.94)
            (8, 0.94)
        };
        \addplot+[forestgreen, no markers, forget plot, line width=1pt] coordinates {
            (-0.5, 0.96)
            (5.5, 0.96)
        };
        \addplot+[dashed, forestgreen, no markers, forget plot, line width=1pt] coordinates {
            (-1, 0.94)
            (5.5, 0.94)
        };
       % \legend{CFG Reward, CFG Result, C-BESO Reward, C-BESO Result}
    \end{axis}

\hspace{0.5cm}
\begin{axis}[
    xlabel=Number Experts,
    at=(abc.right of south east),
    width=4cm,
    ymin=0, ymax=5,
    xmin=4, xmax=8,
    xtick={4,6,8},
    xticklabels={4,6,8},
    yticklabels={0,1,2,3,4,5},
    grid=both,
    grid style={dashed},
    nodes near coords,
    point meta=explicit symbolic,
]
        \addplot+[steelblue, sharp plot,no markers, mark options={solid}, line width=1pt] coordinates {
            (4, 2.3)
            (6, 1.82)
            (8, 1.82)
        };
        \addplot+[crimson, sharp plot, no markers, mark options={solid}, forget plot, line width=1pt] coordinates {
            (3, 3.19)
            (4, 2.74)
            (5, 2.16)
        };
        \addplot+[forestgreen, no markers, forget plot, line width=1pt] coordinates {
            (-0.5, 3.98)
            (5.5, 3.98)
        };
        \addplot+[dashed, forestgreen, no markers, forget plot, line width=1pt] coordinates {
            (-0.5, 3.76)
            (5.5, 3.76)
        };
    \end{axis}
\end{tikzpicture}
